Detecting Alzheimer's Disease Using Gated Convolutional Neural Network from Audio Data

We propose an automatic detection method of Alzheimer's diseases using a gated convolutional neural network (GCNN) from speech data. This GCNN can be trained with a relatively small amount of data and can capture the temporal information in audio paralinguistic features. Since it does not utilize any linguistic features, it can be easily applied to any languages. We evaluated our method using Pitt Corpus. The proposed method achieved the accuracy of 73.6%, which is better than the conventional sequential minimal optimization (SMO) by 7.6 points.

==> sections/experimental_results.tex <==
%!TEX root =  ../main.tex
%%experimental_results%%

\begin{figure}[t]
  \centering
  \includegraphics[width=75mm]{figures/std_cnn_comp.pdf}
%   \includegraphics[width=100mm,scale=0.5]{figures/std_cnn_comp.pdf}
  \caption{Comparison of IS09, IS10, IS11, and IS12 feature sets using standard CNN with sb and ub denote the subject-level and utterance-level based classification respectively.}
  \label{fig:std_cnn_comp}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/uttr_length_stat.pdf}
%   \includegraphics[width=120mm,scale=0.7]{figures/uttr_length_stat.pdf}
  \caption{GCNN with different utterance length.}
  \label{fig:uttr_length_stat}
\end{figure}

\begin{table}[t]
\centering
\caption{Comparison of the employment of the standard CNN and GCNN by using IS10 feature set represented in the average accuracy (\%) from 10-fold cross validation.}
\label{table:all_comparison}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Depth} & \multicolumn{2}{c}{\textbf{Standard CNN}} & \multicolumn{2}{c}{\textbf{Linear GCNN}} \\ 
\textbf{}      & \textbf{Utterance}  & \textbf{Subject}  & \textbf{Utterance}   & \textbf{Subject}  \\ \midrule
1              & 64.2              & 66.0            & 62.2               & 66.2            \\
2              & 64.2              & 66.6            & 62.6               & 68.7            \\
3              & 64.2              & 69.2            & 61.9               & 66.4            \\
4              & 64.9              & 68.7            & 63.3               & 68.9            \\
6              & 65.5              & 68.6            & 65.1               & 72.2            \\
8              & 66.1              & 69.0            & 66.3               & \textbf{73.6}   \\
10             & 65.2              & 70.4            & 65.2               & 69.8            \\ \bottomrule
\end{tabular}
\end{table}

We used the average accuracy from the 10-fold cross validation scheme on Pitt Corpus \cite{becker1994natural} (see Section 3 for details) for evaluating our method. Our first experiment was the employment of the standard deep CNN without gates on the four feature sets, IS09, IS10, IS11, and IS12. Figure \ref{fig:std_cnn_comp} shows the classification result of AD/non AD with different numbers of hidden layers (1, 2, 3, 4, 6, 8, 10). The performance result given is from the subject-level classification after majority voting from the utterance-level classification. Since there is no established baseline for this database and the number of instances used are different from one experiment to another experiment, we give the result of the four feature sets with baseline methods, which is the subject-level classification using sequential minimal optimization (SMO) \cite{schuller2009interspeech,schuller2010interspeech}. In Figure \ref{fig:std_cnn_comp}, they are marked by a star symbol (*). 

%  we can see that the use of IS11 and IS12 yield good results in subject-level classification. However, the employment of CNN on the two feature sets could not improve the classification performance. Contrary to IS09 and IS10, the utilization of the two feature set with CNN yields better results, especially with many layers. When we used IS10, 10-layer CNN is better than SMO by 2.9 points. When we use IS09, 6-layer CNN is better than

From Figure \ref{fig:std_cnn_comp}, the best result is obtained when we use 10-layer CNN with IS10 feature set which is better than SMO by 2.4 points. Furthermore, we can see that the use of CNN with both IS11 and IS12 could not yield better result compared to using SMO while it can improve the performance over using IS09 and IS10. We can also see that the IS10 feature set outperformed the rest of the feature sets when we use CNN.

When we compare between IS09 and IS10, we can see that IS10 covers more features in the paralinguistic aspect of speech as it was used as the age-gender and level-of-interest classification. The performance of the feature sets IS09 was worse than that of IS10 especially when the subjects did not have any specific emotion (neutral). Some emotions appeared at the beginning before the subject begins to describe the image, in the middle when the subject begins to confuse with the things he/she wants to describe (laughs), and at the end after completing the task.

Noticeable differences between IS09 and IS10 include the use of voicing probability in which might more represent the sound-silence pattern in the subjects. Further, jitter and shimmer in IS10 might give more representation of the hesitation rate in the subjects. Those LLD are also appear in both IS11 and IS12. However, the higher dimension of the two feature sets might be too big for the input of the CNN.

% We can also see that the IS10 feature set outperformed IS09 in almost all of the models. This might be because IS10 comprises more features than IS09 as explained in Section \ref{sec:features}. Furthermore, IS10 also covers more features in the paralinguistic aspect of speech as it was used as the age-gender and level-of-interest classification compared to IS09. In addition, we have the voicing probability in IS10 which might more represent the sound-silence pattern in the subjects and also jitter and shimmer which might give more representation of the hesitation rate in the subjects.

Next, we investigated the effectiveness of the gating mechanism. The experiment was carried out by using IS10 feature set. The comparison of the standard CNN and the gating mechanism is shown in Table \ref{table:all_comparison}. From the table, we can see that the employment of linear gate improved the average accuracy from the 10-fold cross validation scheme into 73.6\%. We can see that the gating mechanism yields better result.

Lastly, we investigated the importance of utterance length information in the classification performance. We tried a set of different segment length $L$, which are 500ms, 1000ms, 2000ms, 4000ms, and also 4295ms which is the segment length of the longest utterance in the dataset. In this case, we segmented each subject data into segments with a predetermined length $L$ without taking into consideration the oracle utterance length. Accordingly, the zero padding is added only for the last utterance segment of the subject if its length is less than $L$. The experiment was carried out by using the best scheme from the previous experiment, which is GCNN. We only tried to use the gated CNN with the number of layers as 6, 8, and 10.

As depicted in Figure \ref{fig:uttr_length_stat}, we can see that shorter segment length yields worse results. However, we can still get close results using the utterance length of 4000ms (69.1\%, 70.8\%, and 69.8\% for 6, 8, and 10 layers respectively) compared to the cases when we use the oracle utterance length (72.2\%, 73.6\%, and 69.8\% for 6, 8, and 10 layers respectively). For 10 layers, we got similar result between using the utterance length of 4000ms and the oracle utterance length with 69.8\%. This result suggests that we can use the approach even if we do not have transcription.

==> sections/future_works.tex <==
%!TEX root =  ../main.tex
%%future_works%%

% - Use more data
% - Use other network structures
% - Evaluation of different languages
% - Classification into the severity of the disease
% - Evaluation of the longitudinal study of AD


==> sections/method.tex <==
%!TEX root =  ../main.tex
%%method%%

\begin{figure}[t]
  \centering
%   \includegraphics[width=\linewidth]{figures/framework_ov.pdf}
  \includegraphics[width=80mm,scale=0.5]{figures/framework_ov.pdf}
  \vspace{-1em}
  \caption{GCNN with depth = 1. The kernel window in the convolutional layer is colored in gray.}
  \label{fig:framework_ov}
  \vspace{-1.5em}
\end{figure}

\subsection{Convolutional Neural Network}
\label{sec:cnn}
In this study, assuming that temporal features are well represented in the frame-level features, we employed a Convolutional Neural Network (CNN) \cite{lecun1989backpropagation} as a classifier. A CNN was inspired by the structure of animal visual cortex for perceiving lights \cite{gu2017recent} and has yielded supreme results in an abundance of tasks in the past few years \cite{goodfellow2016deep}. Furthermore, it needs relatively small amount of training data compared to the other networks since it has a much smaller number of connection weights \cite{bengio2009learning}.

The convolution operation over the input aims to extract the temporal information by sliding through the use of a kernel (filter). In our study, we feed utterance segment features \(X \in \R ^ {F \times T}\) into the CNN, where \(F\) and \(T\) represent the dimension of a feature vector of LLD and the number of time frames, respectively. The size of the sliding window is \(\R ^ {F \times N}\) where \(N\) is the window length of the kernel in time axis. The convolution operation between the kernel and the input will produce a scalar output. Output from the convolution layer at time \(i\), \(i = n+1, ..., T\) is then defined as,

\begin{equation}
\label{eq:cnn1}
y_{i} = g\left(\sum\limits_{f = 1}^{F} \sum\limits_{n = 1}^{N} w_{f,n}x_{f,i-n} + b\right),
\end{equation}

\noindent
where \(b\) and \(g\left(\cdot\right)\) denotes the bias and activation function respectively. \(x_{c,d}\) is the \((c,d)\) element of the input \(X\), and \(w_{c,d}\) is the \((c,d)\) element of the weight matrix \(W\). Both \(W\) and \(b\) are the learnable parameters of the network that we train. When the kernel is sliding through the input matrix over the time dimension, we multiply the overlapping element of the two matrices as in Eq. \ref{eq:cnn1}. We employed a rectified linear unit (ReLU) \cite{hahnloser2000digital} as the activation function \(g\). This network is also referred as Time-Delay Neural Network (TDNN) \cite{waibel1990phoneme}.

Since the input dimension for CNN should be fixed, we set the segment length as that of the longest utterance segment in the dataset. After that, we applied zero padding for the rest of the utterance segment. We use the number of kernels \(K = 64\) and the window length of \(N = 3\). Accordingly, the calculation of every patch of the input will produce the complete output \(Y \in \R ^ {M \times K}\) where \(M\) is the number of time frames, \(T - N + 1\).

We added batch normalization before each activation function \cite{ioffe2015batch}. We also used random weight initialization for each convolution layer. After each convolution layer, we put a max-pooling layer \cite{zhou1988computation}. 

The output of the last convolution layer is flattened into one feature vector. For example, the flattened output \(Y \in \R ^ {M \times N}\) will produce a vector \(Z \in \R ^ O\) where \(O = M \times N\). This vector became the input to a fully-connected layer with activation function ReLU consisting 256 hidden neurons. We also employed batch normalization and initialized the weight matrix as random uniform. Furthermore, we also applied dropout with the value of 0.5 before the output layer. The output layer consists one hidden neuron with a sigmoid function. We used binary cross-entropy as the loss function and Adam \cite{kingma2014adam} as the optimizer. We trained the network with the maximum number of epochs 200 based on the pair of LLD features of each utterance segment and its corresponding binary label. 

\subsection{Gating Mechanism}

In addition to the standard deep convolutional neural network, we introduce a gating mechanism after each convolution. The resulting network is called Gated Convolution Neural Network (GCNN). A gate represents an information controller which manages the information that flows into the succeeding layer. The gate function can prevent the gradient from being vanished during backpropagation \cite{dauphin2016language}. Recently, it has been often used in convolutional neural networks such as for conditional image modeling \cite{oord2016conditional}, language modeling \cite{dauphin2016language}, and speech synthesis \cite{oord2016wavenet}. Previous study \cite{dauphin2016language} showed that gated linear unit (GLU) outperformed gated tanh unit (GTU) which is used in \cite{oord2016conditional}. Therefore, we employed GLU in our study.

Similar as in Section \ref{sec:cnn}, we give the input of extracted LLD features of each utterance segment \(X \in \R ^ {T \times F}\). We used a sigmoid function as the activation function \(g\), which is multiplied by a linear gate. Eq. \ref{eq:cnn1} is modified as:

\begin{dmath}
\label{eq:gcnn}
y_i = \left(\sum\limits_{f = 1}^{F} \sum\limits_{n = 1}^{N} v_{f,n}x_{f,i-n} + e\right)
\cdot g\left(\sum\limits_{f = 1}^{F} \sum\limits_{n = 1}^{N} w_{f,n}x_{f,i-n} + b\right),
\end{dmath}

\noindent
where \(v_{c,d}\) represent the element of \(V\) at position \((c,d)\). The \(V \in \R ^ {K \times F}\) and \(e \in \R\) are the kernel weight matrix and bias for the linear gate. For GCNN, we used \(N = 2\) and applied the same padding as in \cite{oord2016wavenet}.

After that, we halved the output length in a max-pooling layer \cite{zhou1988computation}. Figure \ref{fig:framework_ov} shows the visualization of our GCNN with the depth \(= 1\) where the \(depth\) represents the number of gated convolution layers. In the figure, one gated convolution layer lies between the dotted horizontal line which followed by the max-pooling layer. Deeper network consists of more gated convolution layers. We also defined the same layers after the max-pooling layer and used the same number of epochs as in Section \ref{sec:cnn}.

\subsection{Framework Overview}
While we need to classify each subject based on his/her whole data, we performed the classification for each utterance instead. This is based on our assumption that the information about a patient having AD or not can still be obtained from a smaller but appropriate length of a segment. After the utterance-based classification is performed, we make the final verdict for each subject based on the proportion of each class; we classified a subject into AD if he/she has AD percentage above the half. The utterance-level subject classification is expected to give more detailed information about the symptoms while most of the previous studies conducted the subject-level classification \cite{khodabakhsh2015evaluation,fraser2016linguistic,zimmerer2016formulaic,orimaye2017predicting,wankerl2017n,sadeghian2017speech}.
